$^{145}$Ba and $^{145, 146}$La structure from lifetime measurements

The occurrence of octupole shapes in even-mass neutron-rich Ba isotopes has been well established. However, the situation with the odd-mass Ba and odd or odd-odd La nuclei around them is far from settled. In order to shed light on these less-studied isotopes, a fast-timing experiment was performed using GRIFFIN at TRIUMF-ISAC. A wealth of excited-state lifetimes in the 100~ps to few ns range have been measured in $^{144, 145, 146}$Ba and $^{145,146}$La populated in the $\beta^-$ and $\beta^--n$ decay of $^{145,146}$Cs. The results do not allow to draw firm conclusions on the possible octupole deformation of these nuclei but suggest different spin and parity assignments than previous works. This work highlights the need for more detailed study of the odd and odd-odd isotopes in this region to properly understand their structure.

==> notes.tex <==

\textbf{NOTE: } The $^{145}$Ba $7/2^-_1$ lifetime could not be traced. NDDC claims to be quoted in~\cite{Smolanczuk1995}, but I don't find any value and our result does not agree.

Ref.~\cite{Robertson1986} is the only previous beta-decay experiment on Cs-145 to Ba-145.

Ref.~\cite{Biswas2005} has a number of lifetimes on Ba-142 and Ba-144 from spontaneous fission and plunger.

Ref.~\cite{Mach1990} from the great H. Mach has a lot of lifetimes from beta decay in 142-146Ba.

\cite{Mitchell2016} very extensive beta decay experiment on Ba-146

\cite{Bucher2017} coulex on Ba-146

\cite{Jia2007} contains calculations for Ba-145 and La-145


Reflection asymmetry seems to be important in the region https://journals.aps.org/rmp/pdf/10.1103/RevModPhys.68.349 , with a probable maximum at Ba-144. In that same compilation, they claim that enhanced B(E1)>$10^{-4}$~W.u. transitions between positive and negative parity bands and indication of reflection asymmetry. 

https://journals-aps-org.ezproxy.library.ubc.ca/prc/pdf/10.1103/PhysRevC.86.044324 Rejects octupole deformation in the g.s. of Ba-145. They claim a great agreement with a quasy-particle rotor model (QPRM). They also predict a 7/2+ below the 11/2-, that would be key.

Theoretical IBMF calculations: https://journals-aps-org.ezproxy.library.ubc.ca/prc/pdf/10.1103/PhysRevC.97.024317 Maybe contact Nomura for aditional calculations~\cite{Nomura2018} . For example, perfect agreement with the 9/2 -> 5/2 B(E2) transition.

https://journals-aps-org.ezproxy.library.ubc.ca/prc/pdf/10.1103/PhysRevC.54.945 Claims that La-145 has octupole deformation, contrary to theoretical calculations. 

Enhanced B(E1) between parity-doublets is an indication of octupole deformation. From https://academic.oup.com/ptp/article/81/5/1057/1854125
